PROP: Pre-training with Representative Words Prediction for Ad-hoc Retrieval

Recently pre-trained language representation models such as BERT have shown great success when fine-tuned on downstream tasks including information retrieval (IR). However, pre-training objectives tailored for ad-hoc retrieval have not been well explored. In this paper, we propose Pre-training with Representative wOrds Prediction (PROP) for ad-hoc retrieval. PROP is inspired by the classical statistical language model for IR, specifically the query likelihood model, which assumes that the query is generated as the piece of text representative of the "ideal" document. Based on this idea, we construct the representative words prediction (ROP) task for pre-training. Given an input document, we sample a pair of word sets according to the document language model, where the set with higher likelihood is deemed as more representative of the document. We then pre-train the Transformer model to predict the pairwise preference between the two word sets, jointly with the Masked Language Model (MLM) objective. By further fine-tuning on a variety of representative downstream ad-hoc retrieval tasks, PROP achieves significant improvements over baselines without pre-training or with other pre-training methods. We also show that PROP can achieve exciting performance under both the zero- and low-resource IR settings. The code and pre-trained models are available at https://github.com/Albert-Ma/PROP.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> PROP_ Pre-training with Representative Words Prediction for Ad-hoc Retrieval/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> PROP_ Pre-training with Representative Words Prediction for Ad-hoc Retrieval/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> PROP_ Pre-training with Representative Words Prediction for Ad-hoc Retrieval/exp.tex <==
\section{Experiments}
In this section, we conduct experiments to verify the effectiveness of PROP on benchmark collections.
\subsection{Datasets}
We first introduce the two large text corpora for pre-training and five downstream ad-hoc retrieval datasets. 
\subsubsection{Pre-training Corpus}
We use two large document corpora, including English Wikipedia and MS MARCO Document Ranking dataset, to pre-train PROP since (1) They are publicly available and easy to collect; (2) A large collection of documents in these datasets could well support our pre-training method. 

\begin{itemize} [leftmargin=*]
\item \textbf{English Wikipedia} contains tens of millions of documents which has been widely used in many pre-training methods and we download the latest dump\footnote{https://dumps.wikimedia.org/} and extract the text with a public script\footnote{https://github.com/attardi/wikiextractor}.

\item \textbf{MS MARCO Document Ranking dataset} is another large-scale document collection which contains about 4 million available documents. This dataset was used in the TREC Deep Learning Track 2019\footnote{https://microsoft.github.io/TREC-2019-Deep-Learning/} and 2020\footnote{https://microsoft.github.io/TREC-2020-Deep-Learning/}. Documents are extracted from real Web documents using the Bing search engine.
\end{itemize} 

By pre-training PROP on English Wikipedia and MS MARCO Document Ranking dataset respectively, we obtain two types of models denoted as \textbf{PROP$_{\text{Wikipedia}}$} and \textbf{PROP$_{\text{MSMARCO}}$}.  

\begin{table}[t]
\renewcommand{\arraystretch}{1.6}
\setlength\tabcolsep{10pt}
  \caption{Statistics of the ad-hoc retrieval datasets}
  \label{tab:datasets}
  \begin{tabular}{ccccc}
    \toprule
    dataset& \#genre & \#queries & \#documents \\% & \#avg\_len\_d
    \midrule
    Robust04 & news & 250 & 0.5M\\ % & 254
    ClueWeb09-B & web pages & 150 & 50M\\ % & 1,506
    Gov2 & .gov pages & 150 & 25M \\ %& 1,133
    MQ2007 & .gov pages & 1,692 & 25M \\ %& 1,133
    MQ2008 & .gov pages & 784 & 25M \\ %& 1,133
  \bottomrule
\end{tabular}
\end{table}

\subsubsection{Downstream Datasets} To verify the effectiveness of PROP, we conduct experiments on 5 representative ad-hoc retrieval datasets. 

\begin{itemize} [leftmargin=*]
\item \textbf{Robust04} consists of 250 queries and 0.5M news articles, whose topics are collected from TREC 2004 Robust Track.

\item \textbf{ClueWeb09-B} is a large Web collection with 150 queries and over 50M English documents, whose topics are accumulated from TREC Web Track 2009, 2010, and 2011. 

\item \textbf{Gov2} is a crawl of the .gov domain Web pages with 25M documents. We use 150 topic queries that are accumulated from TREC Terabyte Tracks 2004, 2005, and 2006. 

\item \textbf{Million Query Track 2007 (MQ2007)} is a LETOR~\cite{qin2013introducing} benchmark dataset with 1692 queries, which uses the Gov2 Web collection. 

\item \textbf{Million Query Track 2008 (MQ2008)} is another LETOR benchmark dataset with 784 queries, which also leverages the Gov2 Web collection.
\end{itemize} 

Note that ClueWeb09-B is filtered to the set of documents with spam scores in the $60^{th}$ percentile, using the Waterloo Fusion spam scores~\cite{cormack2011efficient}. The detailed statistics of these datasets are shown in Table~\ref{tab:datasets}.
As we can see, there is a significant difference between the number of queries and documents, which poses the challenge of training deep neural models with such a few queries.
Therefore, pre-training on large text corpus to learn universal properties can be beneficial for downstream ad-hoc retrieval tasks and avoid training deep neural model from scratch.


\subsection{Baselines}
We adopt three types of baseline methods for comparison, including traditional retrieve models, pre-trained models, and previous state-of-the-art neural ranking models.

For traditional retrieval models, we take two representative ranking methods:
\begin{itemize} [leftmargin=*]
\item \textbf{QL}: Query likelihood model ~\cite{zhai2017study} is one of the best performing language models based on Dirichlet smoothing. 
\item \textbf{BM25}: The BM25 formula ~\cite{robertson1994some} is another highly effective retrieval model that represents the classical probabilistic retrieval model. 
\end{itemize}

The pre-trained models include:
\begin{itemize} [leftmargin=*]
\item \textbf{BERT}: The key technical innovation of BERT ~\cite{devlin2018bert} is applying the multi-layer bidirectional Transformer encoder architecture for language modeling. BERT uses two different types of pre-training objectives, including Masked Language Model (MLM) and Next Sentence Prediction (NSP). Currently, BERT has become a strong baseline model for ad-hoc retrieval tasks due to its powerful contextual language representations. Different from  passage-level and sentence-level approaches~\cite{dai2019deeper,yang2019simple}, we truncate the single input sequence of the concatenated query and document to BERT's max-length limit.

\item \textbf{Transformer$_{ICT}$}: Inverse Cloze Task (ICT) \cite{lee2019latent} is specifically designed for passage retrieval in QA scenario which teaches model to predict the removed sentence given a context text. As observed in Chang et.al~\cite{chang2020pre}, ICT outperforms BFS and WLP task. Thus, we only choose ICT as the baseline for comparison.
We pre-train the Transformer model on Wikipedia corpus with ICT and MLM for a fair comparison, and other experimental settings are set the same as PROP.


\end{itemize}

Besides the above baselines, we also compare PROP with existing state-of-the-art models (SOTA) on these five datasets, including CEDR-KNRM~\cite{macavaney2019cedr} on Robust04, BERT-maxP~\cite{dai2019deeper} on ClueWeb09-B, NWT~\cite{guo2016semantic} on Gov2, and HiNT~\cite{fan2018modeling} on MQ2007 and MQ2008. We only fetch the best results of these models from the original paper. 
For ClueWeb09-B, previous SOTA BERT-maxP from Dai and Callan \cite{dai2019deeper} used a different set of queries, and thus we use their implementation to run the same query set for comparison. 
%Since CEDR incorporates BERT’s classification vector into existing neural models where can also replace BERT by PROP, we don't include CEDR as our baseline~\cite{macavaney2019cedr}.

\subsection{Evaluation Methodology}
Given the limited number of queries for each collection, we conduct 5-fold cross-validation to minimize overfitting without reducing the number of learning instances. 
The parameters for each model are tuned on 4-of-5 folds. The final fold in each case is used to evaluate the optimal parameters. 
As for evaluation measures, two standard evaluation metrics, i.e., normalized discounted cumulative gain (nDCG) and precision (P), are used in experiments.    
Specifically, for Robust04, ClueWeb09-B and Gov2, we report normalized discounted cumulative gain at rank 20 (NDCG@20) and precision at rank 20 (P@20) following existing works~\cite{dai2019deeper,guo2016deep,macavaney2019cedr}. 
For MQ2007 and MQ2008, we report two official metrics used in LETOR 4.0: precision at rank 10 (P@10) and normalized discounted cumulative gain at rank 10 (NDCG@10) following existing works~\cite{pang2017deeprank,fan2018modeling}, since there are less document candidates for each dataset on the two datasets.
%The statistical significance tests are performed using the paired t-test. Differences are considered statistically significant when the $p-value$ is lower than 0.05.


\subsection{Implementation Details}
Here, we describe the implementation details of PROP, including model architecture, pre-training process and fine-tuning process.

\subsubsection{Model Architecture} We use the Transformer encoder architecture similar to BERT$_{base}$ version \cite{devlin2018bert}, where the number of layers is 12, the hidden size is 768, the feed-forward layer size is 3072, the number of self-attention heads is 12, and the total parameters is 110M. 
For a fair comparison, PROP, BERT and Transformer$_{ICT}$ use the same model architecture in experiment. Specifically, we use the popular transformers library PyTorch-Transformers\footnote{https://github.com/huggingface/transformers} for the implementation of PROP.


\subsubsection{Pre-training Process} 
For representative word sets sampling, the expectation of interval $\lambda$ is set to $3$. 
To avoid sampling frequent words, we perform stopwords removal using the INQUERY stop list, discard the words that occur less than 50 times and use a subsampling of frequent words with sampling threshold of $10^{-5}$ as suggested by Word2Vec\footnote{https://github.com/tmikolov/word2vec}. Word sets are sampled with replacement, i.e. the probability for each word remains the same for multi-sampling.
%, but we omit the duplicate word in the final word set. 
We sample $5$ pairs of word sets for each document.

For the representative words prediction, we lowercase the pre-training text and do not perform stemming or stop words removal. 
The single input sequence which is concatenated by the word set and the document, is fed to PROP. We use Adam optimizer with a linear warm-up over the first 10\% steps and linear decay for later steps, and the learning rate is set to $2e-5$. Dropout with probability of 0.1 is applied on all layers. 
We train with batch size of 128 and sequence length of 512 for about 100-300k steps. 
Considering the large cost of training from scratch, we adopt the parameters of BERT$_{base}$ released by Google\footnote{https://github.com/google-research/bert} to initialize the Transformer encoder. 
We pre-train PROP on 4 Nvidia Telsa V100-32GB GPUs. 

For the masked language modeling, following BERT, we randomly select 15\% words in the input document, and the selected words are (1) 80\% of time replaced by a mask token [MASK], or (2) 10\% of time replaced by a random token, or (3) 10\% of time unchanged. Note that sampled words in representative word sets are not considered to be masked. 



\subsubsection{Fine-tuning Process} 
We adopt a re-ranking strategy for efficient computation. An initial retrieval is performed using the Anserini toolkit with BM25 model to obtain the top 200 ranked documents. We then use PROP to re-rank these top candidate documents.
For all five downstream datasets, we conduct 5-fold cross-validation where each iteration uses three folds for training, one for validation, and a final held-out fold for testing. We employ a batch size among 16 and 32 and select the best fine-tuning learning rate of Adam among $1e-5$ and $2e-5$ on the validation set. 
For Robust04, ClueWeb09-B and Gov2 datasets, we perform the evaluation by using the five folds provided by Huston and Croft~\cite{huston2014parameters}. And for MQ2007 and MQ2008 datasets, we follow the data partition in LETOR4.0~\cite{qin2013introducing}. 
For all pre-trained models including BERT, Transformer$_{ICT}$ and PROP, we use raw text as the input. 
The reason is that using standard stop words removal and words stemming will hurt performance for these pre-trained models in the fine-tuning phase since it is inconsistent with pre-training process. 


\begin{table*}[t]
\renewcommand{\arraystretch}{1.6}
\setlength\tabcolsep{2pt}
  \caption{Comparisons between PROP and the baselines. $\ast, \dag$ and $\ddag$ indicate statistically significance with $p-value \le 0.05$ over $\textbf{BM25}$, $\textbf{BERT}$ and Transformer$_{ICT}$, respectively.}
  \label{tab:main_res1}
  \begin{tabular}{ccccccccccccccc}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{Robust04} & &\multicolumn{2}{c}{ClueWeb09-B} && \multicolumn{2}{c}{Gov2}  && \multicolumn{2}{c}{MQ2007} && \multicolumn{2}{c}{MQ2008}\\
    \cline{2-3} \cline{5-6} \cline{8-9}  \cline{11-12}  \cline{14-15}  
  & nDCG@20 & P@20 & &nDCG@20 & P@20 && nDCG@20 & P@20 && nDCG@10 & P@10&& nDCG@10 & P@10  \\
    \midrule
     QL & 0.413 & 0.367 && 0.225 &0.326 & & 
     0.409 &0.510&&0.423&0.371&&0.223&0.241\\
     %0.465$^{\ddag}$ &0.527$^{\ddag}$\\
    BM25 & 0.412 &0.363& &0.230 & 0.334& &0.421 &0.523&&0.414&0.366&&0.220&0.245\\
    %0.474$^{\ddag}$ &0.534$^{\ddag}$ \\
    Previous SOTA& \textbf{0.538} 
    &\textbf{0.467}&& 0.296& -&& 0.422 & 0.524 && 0.490&
      0.418&&
      0.244&
      0.255\\
    \midrule
      BERT& 0.459$^{\ast}$  & 0.389$^{\ast}$ && 0.295$^{\ast}$& 0.367$^{\ast}$  && 0.495$^{\ast}$& 0.586$^{\ast}$ &&0.506$^{\ast}$&0.419$^{\ast}$&&0.247$^{\ast}$&0.256$^{\ast}$ \\
      Transformer$_{ICT}$ & 0.460$^{\ast}$ & 0.388 $^{\ast}$&& 0.298$^{\ast}$ & 0.369$^{\ast}$ && 0.499$^{\ast\dag}$&0.587$^{\ast}$ && 0.508$^{\ast}$ & 0.420$^{\ast}$ && 0.245$^{\ast}$ & 0.256$^{\ast}$ \\
    \bottomrule
    \tabincell{c}{PROP$_{Wikipedia}$} & \textbf{0.502}$^{\ast\dag\ddag}$& \textbf{0.421}$^{\ast\dag\ddag}$& &
    0.316$^{\ast\dag\ddag}$&
    0.384$^{\ast\dag\ddag}$ &&
    0.519$^{\ast\dag\ddag}$ &
    0.593$^{\ast\dag\ddag}$ &&
    \textbf{0.523}$^{\ast\dag\ddag}$ &
    \textbf{0.432}$^{\ast\dag\ddag}$ &&
    0.262$^{\ast\dag\ddag}$ &
    0.267$^{\ast\dag\ddag}$ 
    \\
    % \hdashline
    \tabincell{c}{PROP$_{MS MARCO}$} &
    0.484$^{\ast\dag\ddag}$ &
    0.408$^{\ast\dag\ddag}$ &&
    \textbf{0.329}$^{\ast\dag\ddag}$ & 
    \textbf{0.391}$^{\ast\dag\ddag}$ && 
    \textbf{0.525}$^{\ast\dag\ddag}$ &
    \textbf{0.594}$^{\ast\dag\ddag}$  &&
    0.522$^{\ast\dag\ddag}$ & 
    0.430$^{\ast\dag\ddag}$ &&
    \textbf{0.266}$^{\ast\dag\ddag}$ & 
    \textbf{0.269}$^{\ast\dag\ddag}$
    \\ 
    \bottomrule
  \end{tabular}
\end{table*}


\subsection{Baseline Comparison}\label{exp}

The performance comparisons between PROP and baselines are shown in Table~\ref{tab:main_res1}. 
We can observe that: 
(1) Traditional retrieval models (i.e., \textit{QL} and \textit{BM25}) are strong baselines which perform pretty well on all downstream tasks. 
(2) By automatically learning text representations and relevance matching patterns between queries and documents, previous state-of-the-art neural ranking models can achieve better results than traditional retrieval models. For Robust04 and ClueWeb09-B, BERT-based models, i.e. CEDR and BERT-maxP, achieve significant improvements over \textit{QL} and \textit{BM25}, while traditional neural ranking models including DRMM and NWT shows slight improvements over \textit{QL} and \textit{BM25} on other three datasets (i.e., Gov2, MQ2007, and MQ2008).   
One possible reason is that it is difficult for a deep neural model training from scratch with such a few supervised pairs.
(3) The improvements of \textit{BERT} and \textit{Transformer$_{ICT}$} over previous \textit{SOTA} on Gov2, MQ2007 and MQ2008 datasets, demonstrate that pre-training and
fine-tuning are helpful for downstream tasks. 
%Although BERT and \textit{Transformer$_{ICT}$} perform really better than previous methods, they are still not the optimal methods for ad-hoc retrieval compared to PROP.

When we look at the two types of \textit{PROP} models pre-trained on Wikipedia and MS MARCO respectively, we find that: \textit{PROP$_{Wikipedia}$} achieves better results than \textit{PROP$_{MSMARCO}$} on Robust04, while \textit{PROP$_{MSMARCO}$} performs better than \textit{PROP$_{Wikipedia}$} on ClueWeb09-B.
The reason might be that the news articles in Robust04 are similar with the well-formed articles in Wikipedia while the Web pages in ClueWeb09-B are similar with the Web documents in MS MARCO. 
%(2) Similar results can also be observed on Gov2, MQ2007 and MQ2008 datasets, where .gov Web pages are aligned better with web documents.
These results suggest that employing the pre-trained model from a related domain for the downstream task is much more effective. 


Finally, we can see that the best \textit{PROP} model achieves the best performance in terms of all the evaluation metrics in 4 of 5 datasets. 
The observations are as follows: 
(1) PROP outperforms traditional retrieval models (i.e., \textit{QL} and \textit{BM25}) by a substantial margin. For example, the relative improvement of \textit{PROP} over \textit{BM25} is about 46\% in terms of nDCG@20 on ClueWeb09-B. 
The results indicate the effectiveness of our pre-training method for ad-hoc retrieval. 
(2) Compared with previous \textit{SOTA}, the relative improvements are about 8.9\%, 24.4\%, 6.7\% and 9\% in terms of nDCG@20 for ClueWeb09-B, Gov2, MQ2007 and MQ2008 respectively. 
For Robust04, CEDR-KNRM is better than PROP since CEDR integrates BERT's representations into existing neural ranking models, e.g. KNRM.
Nevertheless, the results demonstrate that pre-training on a large corpus and then fine-tuning on downstream tasks is better than training a neural deep ranking model from scratch. 
(3) The improvements of PROP over existing pre-trained models (i.e., \textit{BERT} and \textit{Transformer$_{ICT}$}) indicate that designing a pre-training objective tailored for IR with a good theoretical foundation is better than directly applying pre-training objectives from NLP on IR tasks. 

\begin{table}[t]
\renewcommand{\arraystretch}{1.6}
\setlength\tabcolsep{1.pt}
  \caption{Impact of pre-training objectives. $\dag$ indicates statistically significance with $p-value < 0.05$.}
  \label{tab:obj}
  \begin{tabular}{ccccccc}
    \toprule
       \multirow{2}{*}{} & \multicolumn{3}{c}{nDCG@20} &&\multicolumn{2}{c}{nDCG@10}\\
    \cline{2-4} \cline{6-7}
    & Robust04 & ClueWeb09-B & Gov2 && MQ2007 & MQ2008
    \\
    \midrule
    w/ MLM  & 0.467  & 0.306 & 0.503 && 0.511 & 0.249  \\
    w/ ROP  & 0.481$^{\dag}$ & 0.321$^{\dag}$ & 0.519$^{\dag}$ && 0.520$^{\dag}$ & 0.262$^{\dag}$ \\
   w/ ROP+MLM& \textbf{0.484$^{\dag}$} & \textbf{0.329$^{\dag}$}  & \textbf{0.525$^{\dag}$} & & \textbf{0.522$^{\dag}$} & \textbf{0.266$^{\dag}$}\\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Impact of Pre-training Objectives} 
In this section, we investigate the effect of different  pre-training objectives in PROP.  
Specifically, we pre-train the Transformer model with the ROP and MLM objective respectively on MS MARCO under the same experiment settings in PROP. 
As shown in Table~\ref{tab:obj}, we report the nDCG results on 5 downstream tasks. 
We can see that: 
(1) Pre-training with MLM on MS MARCO shows slight improvements over BERT pre-trained on BooksCorpus and English Wikipedia (as shown in Table~\ref{tab:main_res1}). 
It indicates that good representations obtained by MLM may not be sufficient for ad-hoc retrieval tasks. 
(2) Pre-training with ROP achieves significant improvements over MLM on all downstream tasks, showing the effectiveness of ROP tailored for IR. 
(3) By pre-training jointly with the ROP and MLM objective, PROP achieves the best performance on all downstream tasks. 
It indicates that the MLM objective which brings good contextual representations and the ROP objective which resembles the relevance relationship for ad-hoc retrieval tasks can contribute together. 

%\begin{table}[t]
%\renewcommand{\arraystretch}{1.5}
%\setlength\tabcolsep{2.5pt}
%  \caption{Impact of pre-training objectives on Robust04 dataset. $\dag$ and $\ddag$ indicates statistically significance over PROP$_{Robust+MLM}$ with $p-value < 0.05$ and $p-value<0.01$ , respectively.}
%  \label{tab:obj}
%  \begin{tabular}{ccccc}
%    \toprule
%    & nDCG@20 & $\Delta$ & P@20 & $\Delta$ \\
%    \midrule
    %BERT  & 0.459 & - &  0.389  & - \\
%    PROP$_{Robust+MLM}$ & 0.466 & - & 0.391 & - \\
%    PROP$_{Robust+ROP}$& 0.490$^{\dag\ddag}$ & +5.2\%  & 0.407$^{\dag\ddag}$& +4.1\% \\
%   PROP$_{Robust+ROP+MLM}$& \textbf{0.494$^{\dag\ddag}$} & +6\%  & \textbf{0.409$^{\dag\ddag}$} & +5\% \\
%  \bottomrule
%\end{tabular}
%\end{table}
\begin{table*}[t]
\renewcommand{\arraystretch}{1.6}
\setlength\tabcolsep{5pt}
  \caption{Impact of Further Pre-training on Target Tasks. Two-tailed t-tests demonstrate the improvements of PROP with further pre-training to that without further pre-training are statistically significant ($\dag$ indicates $\text{p-value} < 0.05$).}
  \label{tab:fp}
  \begin{tabular}{cccccccc}
    \toprule
    \multirow{2}{*}{} & \multicolumn{3}{c}{nDCG@20} &&\multicolumn{2}{c}{nDCG@10}\\
    \cline{2-4} \cline{6-7}
    & Robust04 & ClueWeb09-B & Gov2 && MQ2007 & MQ2008
    \\
    \midrule
    Without Further Pre-training & 0.502 & 0.329 & 0.525 && 0.523 & 0.266\\
    Further Pre-training & 0.506$^{\dag}$ & 0.334$^{\dag}$ & 0.531$^{\dag}$ &&0.526$^{\dag}$&0.270$^{\dag}$ \\

  \bottomrule
\end{tabular}
\end{table*}

\begin{table}[t]
\renewcommand{\arraystretch}{1.5}
\setlength\tabcolsep{1.5pt}
  \caption{Impact of Different Sampling Strategies. Two-tailed t-tests demonstrate the improvements of document language model-based sampling to the random sampling strategy are statistically significant ($\dag$ indicates $\text{p-value} < 0.05$). }
  \label{tab:ss}
  \begin{tabular}{ccccccc}
    \toprule
   \multirow{2}{*}{} & \multicolumn{3}{c}{nDCG@20} &&\multicolumn{2}{c}{nDCG@10}\\
    \cline{2-4} \cline{6-7}
    & Robust04 & ClueWeb09-B & Gov2 && MQ2007 & MQ2008
    \\
    \midrule
    Random  & 0.471  &0.304 & 0.505 && 0.513 & 0.252  \\
    docLM-based  & 0.493$^{\dag}$ & 0.317$^{\dag}$ & 0.517$^{\dag}$ && 0.516$^{\dag}$ & 0.257$^{\dag}$ \\
  \bottomrule
\end{tabular}
\end{table}


\subsection{Impact of Sampling Strategies}

As described in Section~\ref{sec:pre-method}, the representative word sets are sampled according to the document language model.  
To investigate the impact of different sampling strategies, we compare the document language model-based sampling strategy  (docLM-based sampling for short) with the random sampling strategy, which randomly samples words from the corpus vocabulary independently. 
Specifically, we pre-train the Transformer model on English Wikipedia only with the ROP objective using docLM-based sampling and random sampling respectively. 
The loss curve of the ROP objective over the pre-training steps  using different sampling strategies is depicted in Figure~\ref{fig:ss} (a). 
We can find that PROP based on the docLM-based sampling strategy converges much faster than that based on the random sampling strategy. 





\begin{figure}[t]
	\centering
		\includegraphics[scale=0.28]{sample-strategy.png}
		  \caption{(a) ROP learning curve on Wikipedia over the pre-training steps. (b) The test performance curve on Robust04 in terms of nDCG@20 over the pre-training steps.}
  \label{fig:ss}
\end{figure}



Moreover, we pre-train the Transformer model at most 250K steps for both sampling strategies, and further fine-tune them on the five downstream datasets. 
As shown in Table~\ref{tab:ss}, we report the nDCG@20 results on Robust04, ClueWeb09-B, and Gov2 datasets, and the nDCG@10 results on MQ2007 and MQ2008 datasets. 
We find that PROP based on the docLM-based sampling strategy can achieve significantly better results than that based on the random sampling strategy. 
We also show the test performance curve in terms of nDCG@20 on Robust04 over the pre-training steps in Figure~\ref{fig:ss}(b). We can observe that PROP based on the docLM-based sampling strategy improves the performance much faster than that based on the random sampling strategy. 

All the above results indicate that the docLM-based sampling strategy is a more suitable way than the random sampling strategy to generate representative word sets for a document.
The reason might be that the document language model roots in a good theoretical IR foundation and thus contributes to the efficiency and effectiveness of the pre-training process. 

\subsection{Further Pre-training on Target Tasks}

Here, we analyze the impact of further pre-training on the  document collections in the target tasks to see how much performance could be improved.   
Specifically, we further pre-train PROP$_{Wikipedia}$ on the document collections of Robust04 and MQ2007 respectively, and  PROP$_{MSMARCO}$ on the document collections of ClueWeb09-B, Gov2 and MQ2008 respectively. 
% , with the learning rate as $3e-5$
As shown in Table~\ref{tab:fp}, we can see that PROP with further pre-training on the document collection in the target tasks outperforms that without further pre-training. 
The results demonstrate that further pre-training on the related-domain corpus could improve the ability of PROP and achieve better performance on the downstream tasks, which is  quite consistent with the previous findings \cite{howard2018universal}.  
However, the improvement of further pre-training over without further pre-training on MQ2007 dataset is less than that on other four datasets. 
The reason might be that MQ2007 has much more queries than other datasets, and enough in-domain information can be well captured  during the fine-tuning process. 



\begin{figure*}[t]
	\centering
		\includegraphics[scale=0.5]{few-shot.png}
		  \caption{Fine-tuning with limited supervised data. The solid lines are PROP fine-tuned using 0 (zero shot), 10, 30, 50, and 70 queries for Robust04, ClueWeb09-B and  Gov2 datasets, using 0 (zero shot), 50, 100, 150, and 200 queries for MQ2007 and MQ2008 datasets. The dashed lines are BERT fine-tuned using the full queries.}
  \label{fig:fs}
\end{figure*}



\subsection{Zero- and Low-Resource Settings}
In real-world practice, it is often time-consuming and difficult to collect a large number of relevance labels in IR evaluation.  
To simulate the low-resource IR setting, we pick the first 10, 30, 50, 70 queries from Robust04, ClueWeb09-B, and Gov2, and the first 50, 100, 150, 200 queries from MQ2007 and MQ2008 to fine-tune PROP$_{Wikipedia}$. 
We fine-tune the models with batch size as three different values (i.e., 4, 8, 16), learning rate as two different values (i.e., 1e-5, 2e-5), and pick the checkpoint with the best validation performance. 
As shown in Figure~\ref{fig:fs}, we can find that:  
(1) \textit{PROP} fine-tuned on limited supervised data can achieve comparable performance with BERT fine-tuned on the full supervised datasets in terms of nDCG and Precision. 
For example, PROP fine-tuned with only 30 queries has outperformed BERT on Robust04, ClueWeb09-B, and Gov2 datasets.   
(3) Furthermore, fine-tuning \textit{PROP} with only 10 queries can achieve comparable results with traditional retrieval models (i.e., \textit{QL}and \textit{BM25}) for Robust04, ClueWeb09-B, and Gov2. 
The results demonstrate that by fine-tuning with small numbers of supervised pairs, PROP is able to adapt to the target task quickly. 
(4) Under the zero resource setting, for example, PROP can achieve about 90\% performance of BERT fine-tuned on the full Gov2 dataset in terms of nDCG@20. 


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX
